Searches for resonances in the tb and tc final states at the high-luminosity LHC

We study resonances decaying to one top quark and one additional quark (b or c) at the low- luminosity and high-luminosity 14 TeV LHC and at a future 33 TeV hadron collider in the context of Snowmass 2013. A heavy W boson that preferentially couples to quarks can be found through its decay to tb. A Kaluza-Klein gluon might have a significant branching ratio to tc. The final state in these searches has a lepton and neutrino from a W boson decay plus two jets, at least one of which is b-tagged. We give expected limits as a function of W boson and KKg masses for different collider energy and integrated luminosity options.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = tbres

default: pdf

ps: ${BASENAME}.tex
	latex  -halt-on-error ${BASENAME}
	latex  ${BASENAME}
	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvips -sPAPERSIZE=letter ${BASENAME}.dvi -o ${BASENAME}.ps
	@echo "Output written to ${BASENAME}.ps"

pdf: ${BASENAME}.tex
	pdflatex  -halt-on-error ${BASENAME}
	pdflatex  ${BASENAME}
	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	@echo "Output written to ${BASENAME}.pdf"

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 


